A Fine-grained Interpretability Evaluation Benchmark for Neural NLP

While there is increasing concern about the interpretability of neural models, the evaluation of interpretability remains an open problem, due to the lack of proper evaluation datasets and metrics. In this paper, we present a novel benchmark to evaluate the interpretability of both neural models and saliency methods. This benchmark covers three representative NLP tasks: sentiment analysis, textual similarity and reading comprehension, each provided with both English and Chinese annotated data. In order to precisely evaluate the interpretability, we provide token-level rationales that are carefully annotated to be sufficient, compact and comprehensive. We also design a new metric, i.e., the consistency between the rationales before and after perturbations, to uniformly evaluate the interpretability on different types of tasks. Based on this benchmark, we conduct experiments on three typical models with three saliency methods, and unveil their strengths and weakness in terms of interpretability. We will release this benchmark https://www.luge.ai/#/luge/task/taskDetail?taskId=15 and hope it can facilitate the research in building trustworthy systems.

==> EMNLP 2022/content/Limitations.tex <==
\section{Limitation Discussion}
%如何更好的评估标注的证据，还需要进一步探索
%我们的数据集包含的任务偏少，由于有一些方法和结构是与任务相关的，所以针对同一类型的任务，多加入一些数据集.是否说一下应该加入更多的模型呢
%由于空间限制，一些指标间的具体分析需要给出，如合理性和模型准确率，合理性和忠诚性之间的关系，MAP与扰动类型的关系

We provide a new interpretability evaluation benchmark which contains three tasks with both English and Chinese annotated data. There are three limitations in our work.
\begin{itemize}[leftmargin=*]
\item How to evaluate the quality of human-annotated rationales is still open. We have several annotators to perform quality control based on human intuitions and experiences. Meanwhile, we compare model behaviors on full inputs and human-annotated rationales to evaluate the sufficiency and comprehensiveness of rationales, as shown in Table \ref{tab:rationale_eval} and Table \ref{tab:eval_rationale_more}. However, this manner has damaged the original input distribution and brings uncontrollable factors on model behaviors. Therefore, how to automatically and effectively evaluate the quality of human-annotated rationales should be studied in the future.
\item We find that the interpretability of model architectures and saliency methods vary with tasks, especially with the input form of the task. Thus our benchmark should contain more datasets of each task type ( e.g., single-sentence task, sentence-pair similarity task and sentence-pair inference task) to further verify these findings. And we will build evaluation datasets for more tasks in the future. 
\item Due to space limitation, there is no analysis of the relationships between metrics, e.g., the relationship between plausibility and accuracy, and the relationship between faithfulness and robustness. We will take these analyses in our future work.
\end{itemize}

Finally, we hope more evaluation metrics and analyses are proposed based on our benchmark. And we hope our benchmark can facilitate the research progress of interpertability.


==> EMNLP 2022/content/abstract.tex <==
\begin{abstract}

While there is increasing concern about the interpretability of neural models, the evaluation of interpretability remains an open problem, due to the lack of proper evaluation datasets and metrics. In this paper, we present a novel benchmark to evaluate the interpretability of both neural models and saliency methods. This benchmark covers three representative NLP tasks: sentiment analysis, textual similarity and reading comprehension, each provided with both English and Chinese annotated data. In order to precisely evaluate the interpretability, we provide token-level rationales that are carefully annotated to be sufficient, compact and comprehensive. We also design a new metric, i.e., the consistency between the rationales before and after perturbations, to uniformly evaluate the interpretability on different types of tasks. Based on this benchmark, we conduct experiments on three typical models with three saliency methods, and unveil their strengths and weakness in terms of interpretability. We will release this benchmark\footnote{\url{https://www.luge.ai/\#/luge/task/taskDetail?taskId=15}} and hope it can facilitate the research in building trustworthy systems.

%We also design a new metric, i.e., the consistency between the rationales before and after perturbations, to uniformly evaluate the interpretability of models and saliency methods on different tasks.

\end{abstract}

==> EMNLP 2022/content/conclusion.tex <==
\section{Conclusion}
We propose a new fine-grained interpretability evaluation benchmark, containing token-level rationales, a new evaluation metric and corresponding perturbed examples for three typical NLP tasks, i.e., sentiment analysis, textual similarity and machine reading comprehension.
The rationales in this benchmark meet primary properties that a rationale should satisfy, i.e., sufficiency, compactness and comprehensiveness.
%, we provide a unified interpretability evaluation benchmark.
The experimental results on three models and three saliency methods prove that our benchmark can be used to evaluate interpretability of both models and saliency methods. 
We will release this benchmark and hope it can facilitate progress on several directions, such as better interpretability evaluation metrics and causal analysis of NLP models.
%We hope this benchmark can facilitate progress on several directions, e.g., better interpretability evaluation metrics, causal analysis of NLP models.

==> EMNLP 2022/content/dataset.tex <==
\section{Evaluation Data Construction}
\label{sec:dataset}

As illustrated in Figure \ref{fig:data-workflow}, the construction of our datasets mainly consists of three steps: 1) data collection for each task; 2) perturbed data construction; 3) iterative rationale annotation and checking. 
We first introduce the annotation process, including the annotation criteria for perturbations and rationales. Then we describe our data statistics. In addition, we show other annotation details in Appendix \ref{sec:data_other}.

\begin{figure}[tb]
\centering
\includegraphics[width=0.45\textwidth]{figure/annotation-process.pdf}
\caption{The construction workflow of our datasets.}
\label{fig:data-workflow}
\end{figure}


\subsection{Data Collection}
\label{ssec:data-collection}

In order to provide a general and unified interpretability evaluation benchmark, we construct evaluation datasets for three representative tasks, i.e., sentiment analysis, semantic textual similarity, and machine reading comprehension. Meanwhile, we create both English and Chinese evaluation datasets for each task. 
%In order to provide a general and unified interpretability evaluation benchmark, we construct evaluation datasets for three representative tasks, i.e., sentiment analysis (SA) representing the single-sentence classification task, semantic textual similarity (STS) representing the sentence-pair similarity task, and machine reading comprehension (MRC) representing the long-text comprehension task. Meanwhile, we create both English and Chinese evaluation datasets for each task. 

\textbf{Sentiment Analysis (SA)}, a single-sentence classification task, aims to predict a sentiment label for the given instance. For English, we randomly select 1,500 instances from Stanford Sentiment Treebank (SST) \cite{socher-etal-2013-recursive} dev/test sets, and 400 instances from Movie Reviews \cite{zaidan-eisner-2008-modeling} test set. For Chinese, we randomly sample 60,000 instances from the logs of an open SA API\footnote{\url{https://ai.baidu.com/tech/nlp_apply/sentiment_classify}. Due to the diversity of these logs, we choose instances from these logs for annotation.} with the permission of users. The annotators select instances for annotation (see Appendix \ref{sec:data_other} for details) and label a sentiment polarity for each unlabeled instance. Then 2,000 labeled instances are chosen for building evaluation set.

\textbf{Semantic Textual Similarity (STS)}, a sentence-pair similarity task, is to predict the similarity between two instances. We randomly select 2,000 pairs from Quora Question Pairs (QQP) \cite{wang-etal-2018-glue} and LCQMC \cite{liu-etal-2018-lcqmc} to build English and Chinese evaluation data respectively.

\textbf{Machine Reading Comprehension (MRC)}, a long-text comprehension task, aims to extract an answer based on the question and the corresponding passage. We randomly select 1,500 triples with answers and 500 triples without answers from SQUAD2.0 \cite{rajpurkar-etal-2018-know} and DuReader \cite{he-etal-2018-dureader} for building English and Chinese evaluation set respectively. 

\subsection{Perturbed Data Creation}
\label{ssec:perturbed-creation}

%which claims that a saliency method is faithful if the feature importance it assigns remains consistent with changes that should not change the internal model decision mechanism.  
Recent studies \cite{jacovi-goldberg-2020-towards, ding-koehn-2021-evaluating} claim that a saliency method is faithful if it provides similar rationales for similar inputs and outputs.
Inspired by them, we propose to evaluate the model faithfulness via measuring how consistent its rationales are regarding perturbations that are supposed to preserve the same model decision mechanism.
In other words, under perturbations, a model is considered to be faithful if the change of its rationales is consistent with the change of its prediction.
%That is, perturbations would not influence the internal decision mechanism of the model 
%Consequently, we construct perturbed examples for each original input by slightly modifying it, where the perturbed ones are supposed to preserve the same model decision mechanism with the original input. 
Consequently, we construct perturbed examples for each original input.
%that are supposed to preserve the same model decision mechanism.  

\paragraph{Perturbation Criteria} 
Perturbations should not change the model internal decision mechanism.
We create perturbed examples from two aspects: 1) perturbations do not influence model rationales and predictions; 2) perturbations cause the alterations of rationales and may change predictions. Please note that the influence of perturbations comes from human's basic intuition on model's decision-making mechanism. Based on the literature \cite{jia-liang-2017-adversarial, mccoy-etal-2019-right, ribeiro-etal-2020-beyond}, we define three perturbation types.
\begin{itemize}[leftmargin=*]
\item \textbf{Alteration of dispensable words}. Insert, delete and replace words that should have no effect on model predictions and rationales, e.g., the sentence ``\textit{what are} some reasons to travel alone'' is changed to ``\textit{list} some reasons to travel alone''.
\item \textbf{Alteration of important words}. Replace important words which have an impact on model predictions with their synonyms or related words, such as ``i dislike you'' instead of ``i hate you''. In this situation, the model prediction and rationale should change with perturbations. 
\item \textbf{Syntax transformation}. Transform the syntax structure of an instance without changing its semantics, e.g., ``the customer commented the hotel'' is transformed into ``the hotel is commented by the customer''. In this case, the model prediction and rationale should not be affected. 
\end{itemize}

For each original input, the annotator first selects a perturbation type, then creates a perturbed example according to the definition of this perturbation type. Please note that the annotators can select more than one perturbation type for an original input. 
We ask the annotator to create at least one perturbed example for each original input. And they need to create at least 100 perturbed examples for each perturbation type. For each task, we have two annotators to create perturbed examples and label golden results for these examples, i.e., sentiment label for SA, similarity label for STS and answer for MRC.
According to the perturbation criteria, most of the perturbed examples have the same results as their original ones.
Then we ask the other two annotators to review and modify the created examples and their corresponding results. Since the annotation task in this step is relatively easy, the accuracy of created examples after checking is more than 95\%.

\subsection{Iterative Rationale Annotation Process}
\label{ssec:rationale-annotation}

Given an input and the corresponding golden result, the annotators highlight important input tokens that support the prediction of golden result as the rationale. Then we introduce the rationale criteria and the annotation process used in our work.

\paragraph{Rationale Criteria} 
As discussed in recent studies \cite{lei-etal-2016-rationalizing, yu-etal-2019-rethinking}, a rationale should satisfy the following properties.
\begin{itemize}[leftmargin=*]
\item \textbf{Sufficiency}. A rationale is sufficient if it contains enough information for people to make the correct prediction. In other words, people can make the correct prediction only based on tokens in the rationale.
\item \textbf{Compactness}. A rationale is compact if all of its tokens are indeed required in making a correct prediction. That is to say, when any token is removed from the rationale, the prediction will change or become difficult to make.
\item \textbf{Comprehensiveness}. A rationale is comprehensive if its complements in the input can not imply the prediction, that is, all evidence that supports the output should be labeled as rationales.
%\item \textbf{Understandable}. A rationale is understandable if it is readability and can be understood by humans. Usually, it is clear and coherent. An understandable rationale can improve user trust in model predictions.
\end{itemize}

\paragraph{Annotation Process}
To ensure the data quality, we adopt an iterative annotation workflow, consisting of three steps, as described in Figure \ref{fig:data-workflow}.

\textbf{Step 1: rationale annotation}. Based on human's intuitions on the model decision mechanism, given the input and the corresponding golden result, the ordinary annotators who are college students majoring in languages label all critical tokens to guarantee the rationale's comprehensiveness. Then they organize these tokens into several sets, each of which should be sufficient and compact. That is to say, each set can support the prediction independently. As described in Table \ref{tab:case_intro}, the first example contains three rationale sets, and tokens in the same color belong to the same set. Based on this set form, the rationale satisfies the above three criteria.

\textbf{Step 2: rationale scoring}. Our senior annotators\footnote{They are full-time employees, and have lots of experience in annotating data for NLP tasks.} double-check the annotations by scoring the given rationales according to the annotation criteria. For each rationale set, the annotators rate their confidences for sufficiency and compactness.
The confidences for \textbf{sufficiency} consist of three classes: \textit{can not support result (1)}, \textit{not sure (2)} and \textit{can support result (3)}. 
And the confidences for \textbf{compactness} compose of four classes: \textit{include redundant tokens (1)}, \textit{include disturbances (2)}, \textit{not sure (3)} and \textit{conciseness (4)}. 
Then based on all rationale sets for each input, the annotators rate their confidences for \textbf{comprehensiveness} on a 3-point scale including \textit{not be comprehensive (1)}, \textit{not sure (2)}, \textit{be comprehensive (3)}.
%For understandability, annotators rate their confidences on a 4-point scale including \textit{can not be understood (1)}, \textit{difficult to be understood (2)}, \textit{can be understood (3)} and \textit{easy to be understood (4)}.

A rationale is considered to be of high-quality if its average score on sufficiency, compactness and comprehensiveness is equal to or greater than $3.0$, $3.6$, $2.6$. That is to say, at least two-thirds of the annotators give the highest confidence, and less than one-third of the annotators give the confidence of ``\textit{not sure}''. Then all unqualified data whose average score on a property is lower than the corresponding threshold goes to the next step.

\textbf{Step 3: rationale modification}. Low-quality rationales are shown to the ordinary annotators again. The annotators correct the rationales to meet the properties with scores below the threshold. 
%According to the scores provided in the previous step, the annotators correct the rationales to meet the properties with low scores. 

Then the corrected rationales are scored by senior annotators again. The unqualified data after three loops is discarded. This iterative annotation-scoring process can ensure the data quality.  

%其他细节放在附录：我们初始标注者经过两轮培训
Other annotation details, such as annotator information, annotation training and data usage instructions, are described in Appendix \ref{sec:data_other}.

%dataset statistic
\begin{table}[tb]
\small
\center
\scalebox{0.9}{
\begin{tabular}{l| c c c | c c c}
\toprule
%\hline
\multirow{2}{*}{Tasks} & \multicolumn{3}{c|}{\textbf{English}} & \multicolumn{3}{c}{\textbf{Chinese}} \\
\cline{2-7}
 & Size & RLR & RSN & Size & RLR & RSN\\
\hline
SA & 1,999 & 20.1\% & 2.1 & 2,160 & 27.6\% & 1.4\\
STS & 2,248 & 50.4\% & 1.0 & 2,146 & 66.6\% & 1.0\\
MRC & 1,969 & 10.4\% & 1.0 & 2,315 & 9.8\% & 1.0\\
\bottomrule
\end{tabular}
}
\caption{Overview of our datasets. ``Size'' shows the number of original/perturbed pairs. ``RLR'' represents the ratio of rationale length to its input length. ``RSN'' represents the number of rationale sets in an input. We report the average RLR and RSN over all data.}
\label{tab:data_stas}
\end{table} 

\subsection{Data Statistics}
\label{ssec:data_stas}
We give a comparison between our benchmark and other existing datasets, as shown in Table \ref{tab:exist_data}. Compared with existing datasets, our benchmark contains three NLP tasks with both English and Chinese annotated data. Compared with ERASER which collects seven existing English datasets in its benchmark and provides snippet-level rationales to satisfy sufficiency and comprehensiveness, our benchmark provides token-level rationales and satisfies all three primary properties of rationales.  

%For each task, we create both English and Chinese evaluation datasets. 
Table \ref{tab:data_stas} shows the detailed statistics of our benchmark. We can see that the length ratio and the number of rationales vary with datasets and tasks, where the length ratio affects the interpretability performance on plausibility, as shown in Table \ref{tab:eval_inter_all}. 

Meanwhile, we evaluate the sufficiency of human-annotated rationales by evaluating model performance on rationales, as shown in Table \ref{tab:rationale_eval}. Despite the input construction based on rationales has destroyed the distribution of original inputs, model performance on human-annotated rationales is competitive with that on full inputs, especially on MRC task and Chinese datasets. We can conclude that human-annotated rationales are sufficient. Meanwhile, we give more data analysis in Table \ref{tab:eval_rationale_more}, such as model performance on non-rationales, sufficiency and comprehensiveness scores. 
%We can see that model performance on non-rationales drops rapidly. 
  



\input{table/rationale-evaluate.tex}


==> EMNLP 2022/content/experiments.tex <==
\section{Experiments}
\label{sec:experiment}

\subsection{Experiment Settings}
\label{sec:exp_set}
We implement three widely-used models and three saliency methods. We give brief descriptions of them and leave the implementation details to Appendix \ref{sec:att-extraction}. The source code will be released with our evaluation datasets.

\paragraph{Saliency Methods}
We adopt integrated gradient (\textbf{IG}) method \cite{sundararajan2017axiomatic}, attention-based (\textbf{ATT}) method \cite{jain-wallace-2019-attention} and linear-based (\textbf{LIME}) \cite{ribeiro2016should} method in our experiments. 
IG assigns importance score for each token by integrating the gradient along the path from a defined input baseline to the original input. 
ATT uses attention weights as importance scores, and the acquisition of attention weights depends on the specific model architecture. 
LIME uses the token weights learned by the linear model as importance scores. 
%We adopt three popular saliency methods in our experiments. Integrated gradient (\textbf{IG}) method \cite{sundararajan2017axiomatic} assigns importance score for each token by integrating the gradient along the path from a defined input baseline to the original input. Attention-based (\textbf{ATT}) method \cite{jain-wallace-2019-attention} takes attention scores as token importance scores. The acquisition of attention scores depends on the model architecture. Linear-based (\textbf{LIME}) method \cite{ribeiro2016should} uses a linear model as the interpretation model to approximate the evaluated model locally, and uses the learned token weights as importance scores. 

For each saliency method, we take the top-$k^d$ important tokens to compose the rationale for an input, where $k^d$ is the product of the current input length and the average rationale length ratio of a dataset $d$, as shown by \textit{RLR} in Table \ref{tab:data_stas}. 

\input{table/main-acc-result.tex}

\paragraph{Comparison Models} For each task, we re-implement three typical models with different network architectures and parameter sizes, namely LSTM \cite{hochreiter1997long}, RoBERTa-base and RoBERTa-large \cite{liu2019roberta}. Based on these backbone models, we then fine-tune them with commonly-used datasets of three specific tasks. 
For SA, we select training sets of SST and ChnSentiCorp\footnote{\tiny{\url{https://github.com/pengming617/bert_classification}}} to train models for English and Chinese respectively. For STS, training sets of QQP and LCQMC are used to train English and Chinese models. For MRC, SQUAD2.0 and DuReader are used as training sets for English and Chinese respectively. For each task, we select the best model on the original dev set. 

In order to confirm the correctness of our implementation, Table \ref{tab:eval_acc_all} shows model performances on both original dev/test and our evaluation datasets. We can see that our re-implemented models output close results reported in related works \cite{liu-etal-2018-lcqmc, wang2017machine, liu2019roberta}. 
Meanwhile, the results of Chinese SA and MRC tasks decrease significantly on our evaluation sets. This may be caused by the poor generalization and robustness of the model, as our evaluation datasets contain perturbed examples and Chinese data for SA is not from the ChnSentiCorp dataset.

\input{table/main-inter-result-one-table.tex}

\subsection{Evaluation Results}
\label{ssec:evaluation_result}
Table \ref{tab:eval_inter_all} shows the evaluation results of interpretability from the plausibility and faithfulness perspectives. 
Within the scope of baseline models and saliency methods used in our experiments, there are three main findings. 
First, based on all models and saliency methods used in our experiments, \emph{our metrics for interpretability evaluation, namely token-F1 score and MAP, are more fine and generic}, especially MAP, which applies to all three tasks. 
Second, \emph{IG method performs better on plausibility and ATT method performs better on faithfulness}. Meanwhile, ATT method achieves best performance in sentence-pair tasks.
Third, with all three saliency methods, in these three tasks, \emph{LSTM model is comparable with transformer model (i.e., RoBERTa based model in our experiments) on interpretability}, though LSTM performs worse than transformer in term of accuracy. We think that the generalization ability of LSTM model is weak, leading to low accuracy, even with relatively reasonable rationales.
%That is, high accuracy does not mean high interpretability.
%Third, with different saliency methods, \emph{RoBERTa-base generally performs better than RoBERTa-large on plausibility}, though RoBERTa-large outperforms RoBERTa-base in term of accuracy.
%Third, \emph{there is much room for improvement in the interpretability of long inputs}, as the plausibility decreases along with the decrease of rationale length ratio.

In the following paragraphs, we first give a comparison between our proposed metrics and those used in related studies. Then we give a detailed analysis about the interpretability results of three saliency methods and three evaluated models.

\paragraph{Comparison between Evaluation Metrics}
%We adopt two metrics for plausibility and three metrics for faithfulness.
We report results of token-F1 and IOU-F1 scores for plausibility. The higher the scores, the more plausible the rationales. 
It can be seen that the two metrics have the similar trends in all three tasks with all three saliency methods.
But token-F1 is much precise than IOU-F1, as the IOU-F1 score of a rationale is 1 only if its overlap with ground truth is no less than 0.5 (Equation \ref{equation:iou-f1}).
However, in all three tasks, overlaps of most instances are less than 0.5, especially in the task with a low \textit{RLR}.
%In SA and MRC tasks, the average token-F1 score on all instances is less than 0.5. 
Thus IOU-F1 is too coarse to evaluate token-level rationales.
Instead, token-F1 focuses on evaluating token impact on model predictions, so as to be more suitable for evaluating compact rationales.
%eliminate the influence of dispensable tokens in evaluation, so as to evaluate the compactness of the rationale.

For faithfulness evaluation, we report results of MAP, sufficiency and comprehensiveness scores.
We can see that our proposed MAP is an efficient metric for faithfulness evaluation.
Specifically, it applies to most tasks, especially non-classification tasks. 
Moreover, in the two classification tasks (i.e., SA and STS), with IG and LIME methods, MAP has the same trend as the other two metrics over all three models, which further indicates that MAP can well evaluate the faithfulness of rationales. 
With ATT method, there is no consistent relationship between these three metrics. 
We think this is because the calculations of sufficiency and comprehensiveness scores with ATT method are not accurate and consistent enough. 
For example, in the SA task, from the comparison of three saliency methods with LSTM model, we can see that the rationales extracted by these methods have similar plausibility scores, but the sufficiency score with ATT method is much higher than that with the other two methods. Please note that a low sufficiency score means a sufficient rationale.  
Similarly, in the STS task with RoBERTa-base model, the rationales extracted by ATT method have a higher plausibility score, as well as a higher sufficiency score.
%We think the reasons are in two-fold. First, the rationales extracted by ATT method are more sensitive to perturbations. Second, the prediction probabilities based on rationales and non-rationales are not accurate enough, as the predictions based on non-rationales have gone beyond the standard output space, which affects the calculations of sufficiency and comprehensiveness scores and may lead to uncertain scores. 
Finally, we believe that other metrics can be proposed based on our benchmark.

\paragraph{Evaluation of Saliency Methods}
LIME, which uses a linear model to approximate a DL classification model, is model-agnostic and task-agnostic. It obtains the highest performance on token-F1 and sufficiency scores in SA and STS tasks, as the rationales extracted by it more accurately approximate the decision process of DL models.
But how to better apply LIME to more NLP tasks is very challenging and as the future work.

When comparing IG and ATT, we find ATT performs better on faithfulness and sentence-pair tasks.
In SA and MRC, IG performs better on plausibility and ATT method achieves better results on faithfulness, which is consistent with prior works \cite{jain-wallace-2019-attention, deyoung-etal-2020-eraser}.
In STS, ATT method achieves higher results both on plausibility and faithfulness than IG method. We think this is because the cross-sentence interaction attentions are more important for sentence-pair tasks.
Interestingly, on all three tasks, there is a positive correlation between MAP (faithfulness) and token-F1 (plausibility) with IG method.

%We also compare another two gradient-based methods (see Appendix \ref{sec:other-extraction}) and find that IG consistently performs best on all base models and tasks. 

\paragraph{Evaluation of Models}
While analyzing interpretability of model architectures, we mainly focus on IG and ATT methods, as LIME is model-agnostic.
%Then we analyze the interpretability of model architectures. As LIME is model-agnostic, we mainly focus on IG and ATT methods.
We find that interpretability of model architectures vary with saliency methods and tasks.
%which contributes to model selection.
%And we believe these findings contribute to model selection.

Compared with transformer models, based on IG method, LSTM is competitive on plausibility and performs better on faithfulness in all three tasks. On the contrary, based on ATT method, transformer models outperform LSTM on plausibility and are competitive on faithfulness in STS and MRC tasks. As discussed above, the interaction between inputs is more important in these two tasks.

From the comparison between two transformer models with different parameter sizes, i.e., RoBERTa-base and RoBERTa-large, we find that RoBERTa-base outperforms RoBERTa-large on plausibility with these two saliency methods. Interestingly, for faithfulness evaluation, RoBERTa-base performs better than RoBERTa-large with IG method, and RoBERTa-large performs better than RoBERTa-base with ATT method.

%We believe these findings contribute to model selection.
We believe these findings are helpful to the future work on interpretability.



==> EMNLP 2022/content/introduction.tex <==
\section{Introduction}
\label{sec:intro}

In the last decade, deep learning (DL) has been rapidly developed and has greatly improved various artificial intelligence tasks in terms of accuracy \cite{deng2014deep, litjens2017survey, pouyanfar2018survey}. However, as DL models are black-box systems, their inner decision processes are opaque to users. This lack of transparency makes them untrustworthy and hard to be applied in decision-making applications in fields such as health, commerce and law \cite{fort-couillault-2016-yes}.
%where users often hope to understand the inner decision process for the output.
Consequently, there is a growing interest in explaining the predictions of DL models \cite{simonyan2014deep, ribeiro2016should, alzantot-etal-2018-generating, bastings-etal-2019-interpretable, jiang-etal-2021-alignment}. Accordingly, many evaluation datasets are constructed and the corresponding metrics are designed to evaluate related works \cite{deyoung-etal-2020-eraser, jacovi-goldberg-2020-towards}.

\input{table/example-our.tex}

In order to accurately evaluate model interpretability\footnote{Despite fine-grained distinctions between ``interpretability'' and ``explainability'', we use them interchangeably.} with human-annotated rationales\footnote{In this paper, we focus on highlight-based rationales, which consist of input elements, such as words and sentences, that play a decisive role in the model prediction.} (i.e., evidence that supports the model prediction), many researchers successively propose the properties that a rationale should satisfy, e.g., sufficiency, compactness and comprehensiveness (see Section \ref{ssec:rationale-annotation} for their specific definitions) \cite{kass1988need, fischer1990minimalist, lei-etal-2016-rationalizing, yu-etal-2019-rethinking}. 
However, the existing datasets are designed for different research aims with different metrics, and their rationales do not satisfy all properties needed, as shown in Table \ref{tab:exist_data}, which makes it difficult to track and facilitate the research progress of interpretability.
In addition, all existing datasets are in English.

Meanwhile, many studies focus on designing guidelines and metrics for interpretability evaluation, where plausibility and faithfulness are proposed to measure interpretability from different perspectives \cite{herman2017promise, alvarez2018towards, yang2019evaluating, wiegreffe-pinter-2019-attention, jacovi-goldberg-2020-towards}. 
Plausibility measures how well the rationales provided by models align with human-annotated rationales. With different annotation granularities, token-level and span-level F1-scores are proposed to measure plausibility \cite{deyoung-etal-2020-eraser, mathew2021hatexplain}. 
Faithfulness measures to what extent the provided rationales influence the corresponding predictions. Some studies \cite{yu-etal-2019-rethinking, deyoung-etal-2020-eraser} propose to compare the model's prediction on the full input to its prediction on input masked according to the rationale and its complement (i.e., non-rationale).
However, it is difficult to apply this evaluation method to non-classification tasks, such as machine reading comprehension.
%However, this evaluation method has damaged the original input and brings uncontrollable factors on model predictions.
Furthermore, the model prediction on the non-rationale has gone beyond the standard output scope, e.g., the prediction label on the non-rationale should be neither positive nor negative in the sentiment classification task. 
Thus the metric provided by this method can not generally and may not precisely evaluate the interpretability.

In order to address the above problems, we release a new interpretability evaluation benchmark which provides fine-grained rationales for three tasks and a new evaluation metric for interpretability. 
Our contributions include: 
\begin{itemize}[leftmargin=*]
\item Our benchmark contains three representative tasks in both English and Chinese, i.e., sentiment analysis, semantic textual similarity and machine reading comprehension. Importantly, all annotated rationales meet the requirements of sufficiency, compactness and comprehensiveness by being organized in the set form.
\item To precisely and uniformly evaluate the interpretability of all tasks, we propose a new evaluation metric, i.e., the consistency between the rationales provided on examples before and after perturbation. The perturbations are crafted in a way that will not change the model decision mechanism. This metric measures model fidelity under perturbations and could help to find the relationship between interpretability and other metrics, such as robustness.
\item We give an in-depth analysis based on three typical models with three popular saliency methods, as well as a comparison between our proposed metrics and the existing metrics. The results show that our benchmark can be used to evaluate the interpretability of DL models and saliency methods.
Meanwhile, the results strongly indicate that the research on interpretability of NLP models has much further to go, and we hope our benchmark will do its bit along the way.
\end{itemize}


\input{table/dataset-stas.tex}



==> EMNLP 2022/content/metrics.tex <==
\section{Metrics}
\label{sec:metric}
Following existing studies \cite{deyoung-etal-2020-eraser, ding-koehn-2021-evaluating, mathew2021hatexplain}, we evaluate interpretability from the perspectives of plausibility and faithfulness. Plausibility measures how well the rationales provided by the model agree with human-annotated ones. And faithfulness measures the degree to which the provided rationales influence the corresponding predictions.
%And the faithfulness aims to reflect the accurate reasoning process of the model when making a decision. 

Different from existing work, we adopt \textbf{token-F1} score for plausibility and propose a new metric \textbf{MAP} for faithfulness.

%\paragraph{Plausibility} The plausibility is to measure how well the rationales provided by models agree with human-annotated rationales. We adopt the \textbf{token F1-score} and \textbf{IOU F1-score} as evaluation metrics.
%and we also report the IOU F1-score and AUPRC score proposed in \citet{deyoung2020eraser}.

\textbf{Token F1-score} is defined in Equation \ref{equation:marco-f1}, which is computed by overlapped rationale tokens. Since an instance may contain multiple golden rationale sets, for the sake of fairness, we take the set that has the largest F1-score with the predicted rationale as the ground truth for the current prediction. 
\begin{equation}
\small
\centering
\begin{aligned}
\texttt{Token-F1} &= \frac{1}{N}\sum_{i=1}^N (2 \times \frac{P_i \times R_i}{P_i+R_i}) \\
\texttt{where} \quad P_i&=\frac{|S_i^p \cap S_i^g|}{|S_i^p|} \,\, \texttt{and} \,\, R_i=\frac{|S_i^p \cap S_i^g|}{|S_i^g|}
\end{aligned}
\label{equation:marco-f1}
\end{equation}
where $S_i^p$ and $S_i^g$ represent the rationale set of $i$-th instance provided by models and human respectively; $N$ is the number of instances.

\textbf{MAP} (Mean Average Precision) measures the consistency of rationales under perturbations and is used to evaluate faithfulness. According to the original/perturbed input pair, MAP aims to calculate the consistency of two token lists sorted by token importance score, as defined in Equation \ref{equation:map}. The high MAP indicates the high consistency.
\begin{equation}
\small
\centering
\texttt{MAP} = \frac{\sum_{i=1}^{|X^p|}(\sum_{j=1}^i G(x_j^p, X_{1:i}^o))/i}{|X^p|}
\label{equation:map}
\end{equation}
where $X^o$ and $X^p$ represent the sorted rationale token list of the original and perturbed inputs, according to the token important scores assigned by a specific saliency method. $|X^p|$ represents the number of tokens in $X^p$. $X_{1:i}^o$ consists of top-$i$ important tokens of $X^o$. The function $G(x,Y)$ is to determine whether the token $x$ belongs to the list $Y$, where $G(x,Y)=1 \, \texttt{iff} \, x \in Y$. 

Meanwhile, we also report results of metrics proposed in  \citet{deyoung-etal-2020-eraser}, i.e., IOU F1-score for plausibility, and the joint of sufficiency and comprehensiveness for faithfulness.

\textbf{IOU F1-score} is proposed on span-level rationales, which is the size of token overlap in two sets divided by the size of their union, as shown by $S_i$ in Equation \ref{equation:iou-f1}. A rationale is considered as a match if its $S_i$ is equal to or greater than $0.5$, as illustrated by the $Greater$ function.
\begin{equation}
\small
\centering
\begin{aligned}
\texttt{IOU-F1} &= \frac{1}{N}\sum_{i=1}^N Greater(S_i, 0.5) \\
\texttt{where} \quad S_i &= \frac{|S_i^p \cap S_i^g|}{|S_i^p \cup S_i^g|} 
\end{aligned}
\label{equation:iou-f1}
\end{equation}

%\paragraph{Faithfulness} The faithfulness aims to reflect the accurate reasoning process of the model when making a decision \cite{jacovi2020towards}. 
The joint of \textbf{sufficiency} ($\texttt{Score-Suf}$) and \textbf{comprehensiveness} ($\texttt{Score-Com}$) is shown in Equation \ref{equation:eraser-faithful}. A lower sufficiency score implies the rationale is more sufficient and a higher comprehensiveness score means the rationale is more influential in the prediction. A faithful rationale should have a low sufficiency score and a high comprehensiveness score.
\begin{equation}
\small
\centering
\begin{aligned}
\texttt{Score-Suf} &= \frac{1}{N}\sum_{i=1}^N (F(x_i)_j - F(r_i)_j) \\
\texttt{Score-Com} &= \frac{1}{N}\sum_{i=1}^N (F(x_i)_j - F(x_i \setminus r_i)_j)
\end{aligned}
\label{equation:eraser-faithful}
\end{equation}
where $F(x_i)_j$ represents the prediction probability provided by the model $F$ for class $j$ on the input $x_i$; $r_i$ represents the rationale of $x_i$, and $x_i\setminus{r_i}$ represents its non-rationale. 

 







==> EMNLP 2022/content/related.tex <==
\section{Related Work}
\label{sec:related_work}

As our work provides a new interpretability evaluation benchmark with human-annotated rationales, in this section, we mainly introduce saliency methods for the rationale extraction, interpretability evaluation datasets and metrics.

\paragraph{Saliency Methods} In the post-hoc interpretation research field, saliency methods are widely used to interpret model decisions by assigning a distribution of importance scores over the input tokens to represent their impacts on model predictions \cite{simonyan2014deep, ribeiro2016should, murdoch2018beyond}. 
They are mainly divided into four categories: gradient-based, attention-based, erasure-based and linear-based. In gradient-based methods, the magnitudes of the gradients serve as token importance scores \cite{simonyan2014deep, smilkov2017smoothgrad, sundararajan2017axiomatic}.
Attention-based methods use attention weights as token importance scores \cite{jain-wallace-2019-attention, wiegreffe-pinter-2019-attention}. 
In erasure-based methods, the token importance score is measured by the change of output when the token is removed \cite{li2016understanding, feng-etal-2018-pathologies}.
Linear-based methods use a simple and explainable linear model to approximate the evaluated model behavior locally and use the learned token weights as importance scores \cite{ribeiro2016should, alvarez-melis-jaakkola-2017-causal}. 
These methods have their own advantages and limitations from aspects of computational efficiency, interpretability performance and so on \cite{nie2018theoretical, jain-wallace-2019-attention, de-cao-etal-2020-decisions, sixt2020explanations}. 
%Therefore, a benchmark is needed to evaluate the performance of these methods.

\paragraph{Interpretability Datasets} 
Many datasets with human-annotated rationales have been published for interpretability evaluation, e.g., highlight-based rationales \cite{deyoung-etal-2020-eraser, mathew2021hatexplain}, free-text rationales \cite{camburu2018snli, rajani-etal-2019-explain} and structured rationales \cite{ye-etal-2020-teaching, geva-etal-2021-aristotle}. 
To create high-quality highlight-based rationales, many studies give their views on the properties that a rationale should satisfy. 
\citet{kass1988need} propose that a rationale should be understood by humans.
\citet{lei-etal-2016-rationalizing} point that a rationale should be compact and sufficient, i.e., it is short and contains enough information for a prediction.
\citet{yu-etal-2019-rethinking} introduce comprehensiveness as a criterion, requiring all rationales to be selected, not just a sufficient set.
Although the above criteria have been proposed for highlight rationales, the existing datasets in Table \ref{tab:exist_data} are built with part of them, as they are conducted on different tasks with individual aims.
%Please note that ERASER \cite{deyoung2020eraser} collects several existing datasets, such as e-SNLI \cite{camburu2018snli} and CoS-E \cite{rajani-etal-2019-explain}. Then they manually review and construct snippet-level rationales to make the rationales satisfy sufficiency and comprehensiveness.

\paragraph{Interpretability Metrics} 
For highlight-based rationales, plausibility and faithfulness are often used to measure interpretability from the aspects of human cognition and model fidelity \cite{arras2017relevant, mohseni2018human, weerts2019human}.
%The plausibility measures how much the rationales provided by the model align with human-annotated rationales \cite{yang2019evaluating, deyoung2020eraser, ding2021evaluating}. 
%Since the rationales are provided in different granularity levels, several metrics are proposed to measure the plausibility, such as token F1-Score, IOU (Intersection-Over-Union) F1-Score and AUPRC (Area Under the Precision-Recall curve) score \cite{deyoung2020eraser, mathew2021hatexplain}. The higher the score, the more plausible the model. 
\citet{deyoung-etal-2020-eraser} propose to use IOU (Intersection-Over-Union) F1-score and AUPRC (Area Under the Precision-Recall curve) score to measure plausibility of snippet-level rationales.
\citet{mathew2021hatexplain} use token F1-score to evaluate plausibility of token-level rationales.
\citet{jacovi-goldberg-2020-towards} provide concrete guidelines for the definition and evaluation of faithfulness.
%For faithfulness evaluation, \citet{jacovi2020towards} provide concrete guidelines and claim that human-provided golden labels and human-judgement should not be involved.
\citet{deyoung-etal-2020-eraser} propose to evaluate faithfulness from the perspectives of sufficiency and comprehensiveness of rationales (Equation \ref{equation:eraser-faithful}). 
However, this evaluation manner is only applicable to classification tasks and brings uncontrollable factors to interpretability evaluation.
Thus \citet{yin-etal-2022-sensitivity} propose sensitivity and stability as complementary metrics for faithfulness.
%As illustrated in Section \ref{sec:intro}, this evaluation manner damages the original input and brings other uncontrollable factors for model predictions.
\citet{ding-koehn-2021-evaluating} evaluate faithfulness of saliency methods on natural language models by measuring how consistent the rationales are regarding perturbations. 


In this work, we provide a new interpretability evaluation benchmark, containing fine-grained annotated rationales, a new evaluation metric and the corresponding perturbed examples.
%In this work, we provide a new interpretability evaluation benchmark, containing fine-grained annotated rationales, a new evaluation metric as well as the corresponding perturbed examples.


%Meanwhile, faithfulness is defined to measure how consistent the rationales are regarding perturbations in \citet{ding2021evaluating}.

%However, such coarse-grained annotation fails to further distinguish dispensable words from the snippet rationale. 
%To evaluate rationale extraction methods based on neural language models, \citet{ding2021evaluating} construct four datasets, where two of them are concerned with number agreement of a verb and the other two are concerned with gender agreement of a pronoun.

%\textbf{Learning with rationales}. Some works \cite{lei-etal-2016-rationalizing, jain2020learning} have proved that models can be further improved by learning from the extracted rationales. Most of these works use a two-model setup: one to extract rationales, and one to make a prediction based on rationales. The two models can be trained independently \cite{jain2020learning} or jointly \cite{lei-etal-2016-rationalizing} via REINFORCE \cite{williams1992simple} style optimization.

%Notably, our benchmark contains fine-grained token-level human-annotated rationales, rather than coarse snippet-level annotations. 

%\citet{chang2019game} introduce the notion of class-wise rationales that explains support for different output classes using a game theoretic framework.
%Two-model methods use independent extraction and prediction modules, so as to first extract explanations from the input and then make predictions based on the extracted explanations (\cite{lei-etal-2016-rationalizing, jain2020learning}).
%Saliency methods regard the well-trained model as a black-box and use gradient or attention to extract explanations to reveal the reasons of prediction (\cite{simonyan2014deep, sundararajan2017axiomatic, smilkov2017smoothgrad}).
%Interpretability evaluation is also studied (\cite{belinkov2019analysis, jacovi2020towards, deyoung2020eraser, ding2021evaluating}) from the perspectives of plausibility and faithfulness.


==> EMNLP 2022/table/dataset-stas.tex <==
\begin{table*}[tb]
\small
\renewcommand\tabcolsep{2.5pt}
\centering
\scalebox{0.95} {
\begin{tabular}{l c c c c}
\toprule
\multirow{2}{*}{Datasets} & \multirow{2}{*}{Granularity} & \multicolumn{3}{c}{Properties}\\
\cline{3-5}
 & & Sufficiency & Compactness & Comprehensiveness\\
\hline
e-SNLI$^\star$ \cite{camburu2018snli} & word & \XSolidBrush & \Checkmark & \XSolidBrush \\
HUMMINGBIRD \cite{hayati-etal-2021-bert} & word & \Checkmark$^-$ & \XSolidBrush & -- \\
HateXplain \cite{mathew2021hatexplain} & word & \Checkmark$^-$ & -- & \Checkmark \\
\hline
Movie Reviews$^\star$ \cite{zaidan-eisner-2008-modeling} & snippet & \Checkmark & \XSolidBrush & \XSolidBrush \\
CoS-E$^\star$ \cite{rajani-etal-2019-explain} & snippet & \Checkmark$^-$ & \XSolidBrush & \Checkmark \\
Evidence Inference$^\star$ \cite{lehman-etal-2019-inferring} & snippet & \Checkmark & \XSolidBrush & \XSolidBrush \\
BoolQ$^\star$ \cite{deyoung-etal-2020-eraser} & snippet &  \Checkmark & \XSolidBrush & \Checkmark \\
\hline
WikiQA \cite{yang-etal-2015-wikiqa} & sentence & \Checkmark & \XSolidBrush & -- \\
MultiRC$^\star$ \cite{khashabi-etal-2018-looking} & sentence & \Checkmark & \XSolidBrush & \Checkmark \\
HotpotQA \cite{yang-etal-2018-hotpotqa} & sentence & \Checkmark & \XSolidBrush & \Checkmark \\
FEVER$^\star$ \cite{thorne-etal-2018-fever} & sentence & \Checkmark & \XSolidBrush & -- \\
SciFact \cite{wadden-etal-2020-fact} & sentence & \Checkmark & \XSolidBrush & -- \\
\hline
Ours & word & \Checkmark & \Checkmark & \Checkmark \\
%WikiAttack
%NaturalQuestion
\bottomrule
\end{tabular}
}
\caption{Statistics of existing datasets with highlight-based rationales. The datasets marked with $^\star$ are collected and modified by ERASER \cite{deyoung-etal-2020-eraser}. ERASER manually reviews and constructs snippet-level rationales to make them satisfy sufficiency and comprehensiveness. \Checkmark$^-$ represents the rationale contains key words, but does not contain enough information for the prediction. The value `-' represents the property is not mentioned in the paper.}
\label{tab:exist_data}
\end{table*}


\iffalse
\begin{table*}[tb]
\small
\renewcommand\tabcolsep{2.5pt}
\centering
\scalebox{0.85} {
\begin{tabular}{l  l  l  c c c}
\toprule
\multirow{2}{*}{Datasets} & \multirow{2}{*}{Task} & \multirow{2}{*}{Granularity} & \multicolumn{3}{c}{Properties}\\
\cline{4-6}
 &  &  & Sufficiency & Compactness & Comprehensiveness\\
\hline
Movie Reviews$^\star$ \cite{zaidan-eisner-2008-modeling} & sentiment analysis & snippet & \Checkmark & \XSolidBrush & \XSolidBrush \\
HUMMINGBIRD \cite{hayati-etal-2021-bert} & style classification & word &  \Checkmark$^-$ & \XSolidBrush & -- \\
HateXplain \cite{mathew2021hatexplain} & hate-speech classification & word &  \Checkmark$^-$ & -- & \Checkmark \\
\hline
BoolQ$^\star$ \cite{deyoung-etal-2020-eraser} & reading comprehensive QA & snippet &  \Checkmark & \XSolidBrush & \Checkmark \\
MultiRC$^\star$ \cite{khashabi-etal-2018-looking} & reading comprehensive QA & sentence & \Checkmark & \XSolidBrush & \Checkmark \\
HotpotQA \cite{yang-etal-2018-hotpotqa} & reading comprehensive QA & sentence &  \Checkmark & \XSolidBrush & \Checkmark \\
WikiQA \cite{yang-etal-2015-wikiqa} & open-domain QA & sentence &  \Checkmark & \XSolidBrush & -- \\
CoS-E$^\star$ \cite{rajani-etal-2019-explain} & commonsense QA & snippet &  \Checkmark$^-$ & \XSolidBrush & \Checkmark \\
\hline
Evidence Inference$^\star$ \cite{lehman-etal-2019-inferring} & evidence inference & snippet & \Checkmark & \XSolidBrush & \XSolidBrush \\
e-SNLI$^\star$ \cite{camburu2018snli} & natural language inference & word & \XSolidBrush & \Checkmark & \XSolidBrush \\
\hline
FEVER$^\star$ \cite{thorne-etal-2018-fever} & fact verification & sentence & \Checkmark & \XSolidBrush & -- \\
SciFact \cite{wadden-etal-2020-fact} & fact verification & sentence & \Checkmark & \XSolidBrush & -- \\
\hline
Ours & three tasks & word & \Checkmark & \Checkmark & \Checkmark \\
%WikiAttack
%NaturalQuestion
\bottomrule
\end{tabular}
}
\caption{Statistics of existing datasets with highlight-based rationales. The datasets marked with $^\star$ are collected and modified by ERASER \cite{deyoung-etal-2020-eraser}. ERASER manually reviews and constructs snippet-level rationales to make them satisfy sufficiency and comprehensiveness. \Checkmark$^-$ represents the rationale contains key words, but does not contain enough information for the prediction. The value `-' represents the property is not mentioned in the paper.}
\label{tab:exist_data}
\end{table*}
\fi

==> EMNLP 2022/table/main-acc-result.tex <==
\begin{table}[tb]
\small
\center
\scalebox{0.88} {
\begin{tabular}{l | cc | cc | cc}
\toprule
\multirow{2}{*}{Models} & \multicolumn{2}{c|}{\textbf{SA} (Acc)} & \multicolumn{2}{c|}{\textbf{STS} (Acc)} & \multicolumn{2}{c}{\textbf{MRC} (F1)} \\
 & Ori & Ours & Ori & Ours & Ori & Ours \\
\hline
\multicolumn{7}{c}{\textbf{English} } \\
\cline{1-7}
LSTM & 78.6 & 78.2 & 78.6 & 74.6 & 58.6 & 54.4 \\
RoBERTa-base & 92.1 & 93.8 & 91.5 & 92.7 & 78.4 & 71.7 \\
RoBERTa-large & 91.3 & 95.4 & 91.4 & 93.2 & 83.8 & 76.0 \\
\hline
\multicolumn{7}{c}{\textbf{Chinese}} \\
\cline{1-7}
LSTM & 86.7 & 60.0 & 77.4 & 75.2 & 75.0 & 66.4 \\
RoBERTa-base & 95.1 & 59.8 & 88.1 & 85.5 & 74.4 & 65.8 \\
RoBERTa-large & 95.0 & 62.6 & 88.1 & 86.0 & 77.8 & 67.8 \\
\bottomrule
\end{tabular}
} 
\caption{Conventional performance of base models on three tasks, where ``Acc'' is short for accuracy. The ``Ori'' dev/test set comes from the same dataset as training set. ``Ours'' represents our evaluation datasets.}
\label{tab:eval_acc_all}
\end{table} 

==> EMNLP 2022/table/main-inter-chinese.tex <==
\begin{table*}[tb]
\renewcommand\tabcolsep{2.5pt}
\small
\centering
\scalebox{0.83} {
\begin{tabular}{l | c c c c c | c c c c c | c c c}
\toprule
\multirow{3}{*}{Models + Methods} & \multicolumn{5}{c|}{SA} & \multicolumn{5}{c|}{STS} & \multicolumn{3}{c}{MRC}\\
\cline{2-6} \cline{7-11} \cline{12-14}
 & \multicolumn{2}{c|}{Plausibility} & \multicolumn{3}{c|}{Faithfulness} & \multicolumn{2}{c|}{Plausibility} & \multicolumn{3}{c|}{Faithfulness} &
 \multicolumn{2}{c|}{Plausibility} & 
 \multicolumn{1}{c}{Faithfulness} \\
\cline{2-3} \cline{4-6} \cline{7-8} \cline{9-11} \cline{12-13} \cline{14-14} 
 & Token-F1$\uparrow$ & IOU-F1$\uparrow$ & MAP$\uparrow$ & Suf$\downarrow$ & Com$\uparrow$ & Token-F1 & IOU-F1 & MAP & Suf & Com & Token-F1 & IOU-F1 & MAP \\
\hline
LSTM + IG & 38.2 & 9.8 & 60.6 & -0.131 & 0.707 & 68.2 & 61.5 & 58.6 & 0.336 & 0.419 & 19.9 & 0.6 & 87.1\\
RoBERTa-base + IG & 35.2 & 12.5 & 51.5 & 0.118 & 0.489 & 71.9 & 71.4 & 62.1 & 0.139 & 0.470 & 34.0 & 9.1 & 67.9 \\
RoBERTa-large + IG & 37.9 & 12.9 & 43.6 & 0.123 & 0.381 & 71.8 & 72.0 & 58.1 & 0.251 & 0.547 & 25.2 & 1.7 & 61.9 \\
\hline
LSTM + ATT & 24.0 & 9.8 & 72.6 & 0.171 & 0.225 & 72.7 & 72.1 & 77.3 & 0.110 & 0.359 & 2.7 & 0.0 & 79.6 \\
RoBERTa-base + ATT & 25.7 & 6.0 & 69.5 & 0.191 & 0.320 & 67.2 & 55.4 & 71.3 & 0.201 & 0.399 & 28.5 & 5.3 & 61.4 \\
RoBERTa-large + ATT & 30.7 & 8.2 & 67.9 & 0.173 & 0.248 & 68.0 & 59.8 & 67.0 & 0.251 & 0.547 & 28.5 & 5.5 & 48.8 \\
\hline
LSTM + LIME & 38.6 & 10.1 & 59.4 & -0.130 & 0.701 & 74.8 & 79.0 & 65.9 & -0.015 & 0.411 & - & - & - \\
RoBERTa-base + LIME & 37.3 & 14.3 & 56.6 & 0.051 & 0.660 & 77.3 & 83.2 & 74.8 & -0.041 & 0.494 & - & - & - \\
RoBERTa-large + LIME & 39.0 & 14.5 & 53.0 & -0.013 & 0.653 & 76.8 & 82.9 & 74.3 & -0.024 & 0.562 & - & - & - \\
\bottomrule
\end{tabular}
}
\caption{Interpretability evaluation results on Chinese datasets of three tasks.} 
\label{tab:eval_inter_chinese}
\end{table*} 


==> EMNLP 2022/table/main-inter-result-one-table.tex <==
\begin{table*}[tb]
\renewcommand\tabcolsep{2.5pt}
\small
\centering
\scalebox{0.83} {
\begin{tabular}{l | c c c c c | c c c c c | c c c}
\toprule
\multirow{3}{*}{Models + Methods} & \multicolumn{5}{c|}{SA} & \multicolumn{5}{c|}{STS} & \multicolumn{3}{c}{MRC}\\
\cline{2-6} \cline{7-11} \cline{12-14}
 & \multicolumn{2}{c|}{Plausibility} & \multicolumn{3}{c|}{Faithfulness} & \multicolumn{2}{c|}{Plausibility} & \multicolumn{3}{c|}{Faithfulness} &
 \multicolumn{2}{c|}{Plausibility} & 
 \multicolumn{1}{c}{Faithfulness} \\
\cline{2-3} \cline{4-6} \cline{7-8} \cline{9-11} \cline{12-13} \cline{14-14} 
 & Token-F1$\uparrow$ & IOU-F1$\uparrow$ & MAP$\uparrow$ & Suf$\downarrow$ & Com$\uparrow$ & Token-F1 & IOU-F1 & MAP & Suf & Com & Token-F1 & IOU-F1 & MAP \\
\hline
LSTM + IG & 36.9 & 12.1 & 67.2 & -0.025 & 0.708 & 54.1 & 17.3 & 69.0 & 0.048 & 0.441 & 40.7 & 11.0 & 72.3 \\
RoBERTa-base + IG & 37.4 & 10.4 & 64.1 & 0.059 & 0.392 & 52.9 & 24.2 & 65.3 & 0.153 & 0.478 & 42.1 & 11.0 & 66.9 \\
RoBERTa-large + IG & 35.0 & 7.9 & 40.6 & 0.130 & 0.260 & 52.7 & 35.9 & 49.7 & 0.224 & 0.400 & 18.0 & 0.1 & 18.0 \\
\hline
LSTM + ATT & 36.6 & 12.4 & 67.8 & 0.123 & 0.298 & 49.6 & 11.8 & 76.0 & 0.221 & 0.313 & 19.9 & 0.4 & 88.3 \\
RoBERTa-base + ATT & 33.2 & 9.4 & 69.2 & 0.267 & 0.128 & 66.5 & 54.2 & 73.6 & 0.185 & 0.337 & 22.6 & 2.6 & 55.0 \\
RoBERTa-large + ATT & 23.3 & 3.1 & 75.9 & 0.301 & 0.095 & 56.8 & 35.9 & 75.4 & 0.136 & 0.399 & 26.6 & 1.3 & 76.0 \\
\hline
LSTM + LIME & 36.6 & 11.3 & 63.2 & -0.040 & 0.762 & 54.5 & 19.2 & 60.0 & 0.134 & 0.311 & - & - & - \\
RoBERTa-base + LIME & 41.5 & 13.8 & 61.0 & 0.032 & 0.568 & 58.7 & 34.9 & 70.5 & 0.064 & 0.509 & - & - & - \\
RoBERTa-large + LIME & 41.4 & 14.3 & 62.9 & 0.053 & 0.505 & 61.2 & 42.3 & 71.8 & 0.019 & 0.524 & - & - & - \\
\bottomrule
\end{tabular}
}
\caption{Interpretability evaluation results on English datasets of three tasks. The metric with $\uparrow$ means the higher the score, the better the performance. Conversely, $\downarrow$ means a low score represents a good performance. As LIME is specially designed for classification tasks, we have not applied it to MRC. Meanwhile, the sufficiency score ($\texttt{Suf}$) and the comprehensiveness score ($\texttt{Com}$) are also only suitable for classification tasks, as shown in Equation \ref{equation:eraser-faithful}. Thus we do not report these two scores on MRC.}
\label{tab:eval_inter_all}
\end{table*} 

%As MRC is a sequence labeling task, it is difficult to compute the sufficiency score and comprehensiveness score, all of which depend on the classification probability, as shown in Equation \ref{equation:eraser-faithful}. Thus we do not report these two scores on the MRC task.
%See Table \ref{tab:eval_inter_english} for English results.}

==> EMNLP 2022/table/rationale-evaluate.tex <==
\begin{table}[tb]
\small
\center
\scalebox{0.83} {
\begin{tabular}{l | cc | cc | cc}
\toprule
\multirow{2}{*}{Models} & \multicolumn{2}{c|}{\textbf{SA}} & \multicolumn{2}{c}{\textbf{STS}} & \multicolumn{2}{c}{MRC} \\
 & Acc$^f$ & Acc$^r$ & Acc$^f$ & Acc$^r$ & F1$^{f}$ & F1$^{r}$\\
\hline
\multicolumn{7}{c}{\textbf{English} } \\
\cline{1-7}
LSTM & 78.2 & \textbf{86.2} & 74.6 & 69.8 & 54.4 & 53.4 \\
RoBERTa-base & 93.8 & 92.4 & 92.7 & 89.3 & 71.7 & \textbf{80.8} \\
RoBERTa-large & 95.4 & 91.5 & 93.2 & 88.8 & 76.0 & \textbf{76.7} \\
\hline
\multicolumn{7}{c}{\textbf{Chinese}} \\
\cline{1-7}
LSTM & 60.0 & \textbf{70.4} & 75.2 & \textbf{80.7} & 66.4 & \textbf{82.2} \\
RoBERTa-base & 59.8 & \textbf{77.0} & 85.5 & \textbf{88.1} & 65.8 & \textbf{89.3} \\
RoBERTa-large & 62.6 & \textbf{80.6} & 86.0 & \textbf{87.4} & 67.8 & \textbf{83.3} \\
\bottomrule
\end{tabular}
} 
\caption{Model performance on the original full input (Acc$^f$) and  human-annotated rationale (Acc$^r$).}
\label{tab:rationale_eval}
\end{table}

\iffalse
\begin{table}[tb]
\small
\center
\scalebox{0.70} {
\begin{tabular}{l | ccc | ccc | cc}
\toprule
\multirow{2}{*}{Models} & \multicolumn{3}{c|}{\textbf{SA}} & \multicolumn{3}{c}{\textbf{STS}} & \multicolumn{2}{c}{MRC} \\
 & Acc$^f$ & Acc$^r$ & Acc$^{nr}$ & Acc$^f$ & Acc$^r$ & Acc$^{nr}$ & F1$^f$ & F1$^r$\\
\hline
\multicolumn{9}{c}{\textbf{English} } \\
\cline{1-9}
LSTM & 78.2 & 86.2 & 60.7 & 74.6 & 69.8 & 61.3 & 54.4 & -\\
RoBERTa-base & 93.8 & 92.4 & 70.6 & 92.7 & 89.3 & 54.8 & 71.7 & 80.8\\
RoBERTa-large & 95.4 & 91.5 & 74.4 & 93.2 & 88.8 & 53.9 & 76.0 & 76.7 \\
\hline
\multicolumn{9}{c}{\textbf{Chinese}} \\
\cline{1-9}
LSTM & 60.0 & 70.4 & 48.7 & 75.2 & 80.7 & 51.2 & 66.4 & -\\
RoBERTa-base & 59.8 & 77.0 & 50.2 & 85.5 & 88.1 & 48.8 & 65.8 & 89.3\\
RoBERTa-large & 62.6 & 80.6 & 47.6 & 86.0 & 87.4 & 48.9 & 67.8 & 83.3\\
\bottomrule
\end{tabular}
} 
\caption{Model performance on the original full input (Acc$^f$), human-annotated rationale (Acc$^r$), and non-rationale (Acc$^{nr}$) by removing human-annotated rationale from the original full input.}
\label{tab:rationale_eval_old}
\end{table}
\fi
